Multivariate Gini-type discrepancies

Measuring distances in a multidimensional setting is a challenging problem, which appears in many fields of science and engineering. In this paper, to measure the distance between two multivariate distributions, we introduce a new measure of discrepancy which is scale invariant and which, in the case of two independent copies of the same distribution, and after normalization, coincides with the scaling invariant multidimensional version of the Gini index recently proposed in [34]. A byproduct of the analysis is an easy-to-handle discrepancy metric, obtained by application of the theory to a pair of Gaussian multidimensional densities. The obtained metric does improve the standard metrics, based on the mean squared error, as it is scale invariant. The importance of this theoretical finding is illustrated by means of a real problem that concerns measuring the importance of Environmental, Social and Governance factors for the growth of small and medium enterprises.

==> tables/table_StatClass32alpha05.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Index & Mean & Median & Variance & MAD & MAX \\
\hline
at3p & 0.253 & 0.235 & 0.015 & 0.007 & 1.064 \\
at3pT1.1 & 0.253 & 0.235 & 0.015 & 0.007 & 1.064 \\
at3pT1.6 & 0.253 & 0.235 & 0.015 & 0.007 & 1.064 \\
at3pT2.2 & 0.253 & 0.235 & 0.015 & 0.007 & 1.064 \\
at3pT2.8 & 0.253 & 0.235 & 0.015 & 0.007 & 1.064 \\
at3pT3.3 & 0.253 & 0.235 & 0.015 & 0.007 & 1.064 \\
atNT1.1 & 0.076 & 0.073 & 0.000 & 0.004 & 0.103 \\
atNT1.6 & 0.082 & 0.080 & 0.000 & 0.005 & 0.115 \\
atNT2.2 & 0.117 & 0.120 & 0.000 & 0.010 & 0.153 \\
atNT2.8 & 0.158 & 0.159 & 0.000 & 0.007 & 0.200 \\
atNT3.3 & 0.242 & 0.239 & 0.000 & 0.012 & 0.268 \\
atST1.1 & 0.047 & 0.041 & 0.000 & 0.001 & 0.091 \\
atST1.6 & 0.052 & 0.047 & 0.000 & 0.002 & 0.086 \\
atST2.2 & 0.073 & 0.065 & 0.000 & 0.005 & 0.094 \\
atST2.8 & 0.088 & 0.091 & 0.000 & 0.008 & 0.105 \\
atST3.3 & 0.116 & 0.116 & 0.000 & 0.005 & 0.132 \\
ea3pT1.1 & 0.481 & 0.478 & 0.025 & 0.109 & 0.917 \\
ea3pT1.6 & 0.351 & 0.328 & 0.017 & 0.084 & 0.716 \\
ea3pT2.2 & 0.241 & 0.218 & 0.011 & 0.064 & 0.538 \\
ea3pT2.8 & 0.153 & 0.138 & 0.007 & 0.048 & 0.392 \\
ea3pT3.3 & 0.089 & 0.072 & 0.004 & 0.033 & 0.274 \\
eaNT1.1 & 0.498 & 0.480 & 0.030 & 0.107 & 0.964 \\
eaNT1.6 & 0.381 & 0.355 & 0.024 & 0.091 & 0.791 \\
eaNT2.2 & 0.286 & 0.251 & 0.018 & 0.078 & 0.645 \\
eaNT2.8 & 0.210 & 0.169 & 0.014 & 0.060 & 0.528 \\
eaNT3.3 & 0.153 & 0.110 & 0.010 & 0.049 & 0.433 \\
eaST1.1 & 0.481 & 0.478 & 0.025 & 0.109 & 0.917 \\
eaST1.6 & 0.351 & 0.328 & 0.017 & 0.084 & 0.716 \\
eaST2.2 & 0.241 & 0.218 & 0.011 & 0.064 & 0.538 \\
\hline
\end{tabular}
\end{table}

